Quasi-Isometries for certain Right-Angled Coxeter Groups

We construct the JSJ tree of cylinders $T_c$ for finitely presented, one-ended, two-dimensional right-angled Coxeter groups (RACGs) splitting over two-ended subgroups in terms of the defining graph of the group, generalizing the visual construction by Dani and Thomas given for hyperbolic RACGs. Additionally, we prove that $T_c$ has two-ended edge stabilizers if and only if the defining graph does not contain a certain subdivided $K_4$. By use of the structure invariant of $T_c$ introduced by Cashen and Martin, we obtain a quasi-isometry-invariant of these RACGs, essentially determined by the defining graph. Furthermore, we refine the structure invariant to make it a complete quasi-isometry-invariant in case the JSJ decomposition of the RACG does not have any rigid vertices.

==> ParkingLot.tex <==
@article{JSJDecompGps,
	Author = {Guirardel, Vincent and Levitt, Gilbert},
	Date-Added = {2020-03-20 14:35:34 +0100},
	Date-Modified = {2020-03-20 14:35:34 +0100},
	Fjournal = {Ast\'{e}risque},
	Isbn = {978-2-85629-870-1},
	Issn = {0303-1179},
	Journal = {Ast\'{e}risque},
	Number = {395},
	Pages = {vii+165},
	Title = {J{SJ} decompositions of groups},
	Year = {2017}}

@article{DaniThomasBowditch,
  title={Bowditch's {JSJ} tree and the quasi-isometry classification of certain {C}oxeter groups},
  author={Dani, Pallavi and Thomas, Anne},
  journal={Journal of Topology},
  volume={10},
  number={4},
  pages={1066--1106},
  year={2017},
  publisher={Wiley Online Library}
}


@article{CashenMartinStructureInvar,
  	Author = {Christopher H. Cashen and Alexandre Martin},
	Date-Added = {2020-03-20 14:35:34 +0100},
	Date-Modified = {2020-03-20 14:35:34 +0100},
	Doi = {10.1017/S0305004116000530},
	Eprint = {1601.07147},
	Journal = {Math. Proc. Cambridge Philos. Soc.},
	Number = {2},
	Pages = {249--291},
	Title = {Quasi-isometries Between Groups with Two-Ended Splittings},
	Volume = {162},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1017/S0305004116000530}}

@book{DavisCoxeter,
  title={The Geometry and Topology of {C}oxeter Groups},
  author={Davis, Michael},
  year={2012},
  publisher={Princeton University Press}
}

@article{MihalikTschantzVisual,
  title={Visual decompositions of {C}oxeter groups},
  author={Mihalik, Michael and Tschantz, Steven},
  journal={Groups, Geometry, and Dynamics},
  volume={3},
  number={1},
  pages={173--198},
  year={2009}
}

@article{GuirardelLevittToC,
  title={Trees of cylinders and canonical splittings},
  author={Guirardel, Vincent and Levitt, Gilbert},
  journal={Geometry \& Topology},
  volume={15},
  number={2},
  pages={977--1012},
  year={2011},
  publisher={Mathematical Sciences Publishers}
}

@article{BowditchJSJtree,
  title={Cut points and canonical splittings of hyperbolic groups},
  author={Bowditch, Brian H.},
  journal={Acta mathematica},
  volume={180},
  number={2},
  pages={145--186},
  year={1998},
  publisher={Springer}
}

@article{Paris1997commensurators,
  title={Commensurators of parabolic subgroups of {C}oxeter groups},
  author={Paris, Luis},
  journal={Proceedings of the American Mathematical Society},
  volume={125},
  number={3},
  pages={731--738},
  year={1997}
}

@book{Sta71,
	Address = {New Haven, Conn.},
	Author = {Stallings, John R.},
	Date-Added = {2020-03-20 14:35:34 +0100},
	Date-Modified = {2020-03-20 14:35:34 +0100},
	Pages = {v+65},
	Publisher = {Yale University Press},
	Title = {Group theory and three-dimensional manifolds},
	Year = {1971},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=0415622}
}
%Mrclass = {57A10 (20E30)}, Mrnumber = {0415622 (54 \#3705)}, Mrreviewer = {Edward M. Bloomberg}, Note = {A James K. Whittemore Lecture in Mathematics given at Yale University, 1969, Yale Mathematical Monographs, 4},

@book{BogopolskiOleg2008Itgt,
  title={Introduction to group theory},
  author={Bogopol'skij, Oleg Vladimirovi{\v{c}}},
  volume={6},
  year={2008},
  publisher={European Mathematical Society}
}
%url={ http://dec1.sinp.msu.ru/~panov/LibBooks/GROUPS/Oleg_Bogopolski-Introduction_to_Group_Theory_%28EMS_Textbooks_in_Mathematics%29-European_Mathematical_Society%282008%29.pdf }


@book{loeh2017geometric,
  title={Geometric group theory},
  author={L{\"o}h, Clara},
  year={2017},
  publisher={Springer}
}

@article{barrett2018computing,
  title={Computing {JSJ} decompositions of hyperbolic groups},
  author={Barrett, Benjamin},
  journal={Journal of Topology},
  volume={11},
  number={2},
  pages={527--558},
  year={2018},
  publisher={Wiley Online Library}
}

@article{RipsE1997CSoF,
issn = {0003-486X},
abstract = {We borrow the Jaco-Shalen-Johannson notion of characteristic submanifolds from 3-dimensional topology to study cyclic splittings of finitely presented groups. The canonical J{SJ} decomposition we construct generalizes the one introduced in [Se1] for (Gromov) hyperbolic groups.},
journal = {Annals of Mathematics},
pages = {53--109},
volume = {146},
publisher = {Princeton University Press},
number = {1},
year = {1997},
title = {Cyclic Splittings of Finitely Presented Groups and the Canonical {JSJ} Decomposition},
copyright = {Copyright 1997 Princeton University},
language = {eng},
address = {PRINCETON},
author = {Rips, Eliyahu and Sela, Zlil},
keywords = {Integers ; Algebra ; Mathematical theorems ; Geometric planes ; Klein bottles ; Euclidean space ; Real lines ; Automorphisms ; Vertices ; Physical Sciences ; Mathematics ; Science & Technology},
}

@article{fujiwara2006jsj,
  title={J{SJ}-decompositions of finitely presented groups and complexes of groups},
  author={Fujiwara, Koji and Papasoglu, Panos},
  journal={Geometric \& Functional Analysis GAFA},
  volume={16},
  number={1},
  pages={70--125},
  year={2006},
  publisher={Springer}
}

@article{papasoglu2005quasi,
  title={Quasi-isometry invariance of group splittings},
  author={Papasoglu, Panos},
  journal={Annals of Mathematics},
  volume={161},
  pages={759--830},
  year={2005},
  publisher={JSTOR}
}

@book{SerreJeanPierre1980T,
  title={Trees and Amalgams},
  author={Serre, Jean-Pierre},
  booktitle={Trees},
  pages={1--68},
  year={1980},
  publisher={Springer}
}

@article{behrstockNeumann,
  title={Quasi-isometric classification of graph manifold groups},
  author={Behrstock, Jason A. and Neumann, Walter D.},
  journal={Duke Mathematical Journal},
  volume={141},
  number={2},
  pages={217--240},
  year={2008},
  publisher={Duke University Press}
}

@article{dani2018commensurability,
  title={Commensurability for certain right-angled {C}oxeter groups and geometric amalgams of free groups},
  author={Dani, Pallavi and Stark, Emily and Thomas, Anne},
  journal={Groups, Geometry, and Dynamics},
  volume={12},
  number={4},
  pages={1273--1341},
  year={2018}
}

@article{cashenmacura,
  title={Line patterns in free groups},
  author={Cashen, Christopher H. and Macura, Nata{\v{s}}a},
  journal={Geometry \& Topology},
  volume={15},
  number={3},
  pages={1419--1475},
  year={2011},
  publisher={Mathematical Sciences Publishers}
}

@article{margolis2018quasi,
  title={Quasi-isometry classification of right-angled Artin groups that split over cyclic subgroups},
  author={Margolis, Alexander},
  journal={Groups, Geometry, and Dynamics},
  volume={14},
  number={4},
  pages={1351--1417},
  year={2020}
}

@inproceedings{gromov1984infinite,
  title={Infinite groups as geometric objects},
  author={Gromov, Mikhael},
  booktitle={Proceedings of the International Congress of Mathematicians},
  volume={1},
  pages={2},
  year={1984}
}

@article{coxeter1934discrete,
  title={Discrete groups generated by reflections},
  author={Coxeter, Harold S. M.},
  journal={Annals of Mathematics},
  pages={588--621},
  year={1934},
  volume={35},
  publisher={JSTOR}
}

@article{papasogluwhyte,
  title={Quasi-isometries between groups with infinitely many ends},
  author={Papasoglu, Panos and Whyte, Kevin},
  journal={Commentarii Mathematici Helvetici},
  volume={77},
  number={1},
  pages={133--144},
  year={2002},
  publisher={Springer}
}

@article{dunwoody1985accessibility,
  title={The accessibility of finitely presented groups},
  author={Dunwoody, Martin J.},
  journal={Inventiones mathematicae},
  volume={81},
  number={3},
  pages={449--457},
  year={1985},
  publisher={Springer}
}

@article{shepherd2020quasi,
  title={Quasi-isometric rigidity for graphs of virtually free groups with two-ended edge groups},
  author={Shepherd, Sam and Woodhouse, Daniel J.},
  journal={arXiv preprint arXiv:2007.10034},
  pages={1--53},
  year={2020}
}

@article{bounds2020quasi,
  title={Quasi-isometric rigidity of a class of right-angled {C}oxeter groups},
  author={Bounds, Jordan and Xie, Xiangdong},
  journal={Proceedings of the American Mathematical Society},
  volume={148},
  number={2},
  pages={553--568},
  year={2020}
}

@article{dani2018large,
  title={The large-scale geometry of right-angled {C}oxeter groups},
  author={Dani, Pallavi},
  journal={arXiv preprint arXiv:1807.08787},
  pages={1--29},
  year={2018}
}

@article{hruska2020surface,
  title={Surface group amalgams that (don't) act on 3-manifolds},
  author={Hruska, G. Christopher and Stark, Emily and Tran, Hung Cong},
  journal={American Journal of Mathematics},
  volume={142},
  number={3},
  pages={885--921},
  year={2020},
  publisher={Johns Hopkins University Press}
}

@article {DaniThomasDiv,
    AUTHOR = {Dani, Pallavi and Thomas, Anne},
     TITLE = {Divergence in right-angled {C}oxeter groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {367},
      YEAR = {2015},
    NUMBER = {5},
     PAGES = {3549--3577},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {20F65 (20F55)},
  MRNUMBER = {3314816},
MRREVIEWER = {Kevin\ D.\ Schreve},
       DOI = {10.1090/S0002-9947-2014-06218-1},
       URL = {https://doi.org/10.1090/S0002-9947-2014-06218-1},
}

@article {BehrstockCFS,
    AUTHOR = {Behrstock, Jason and Falgas-Ravry, Victor and Hagen, Mark F.
              and Susse, Tim},
     TITLE = {Global structural properties of random graphs},
   JOURNAL = {Int. Math. Res. Not. IMRN},
  FJOURNAL = {International Mathematics Research Notices. IMRN},
      YEAR = {2018},
    NUMBER = {5},
     PAGES = {1411--1441},
      ISSN = {1073-7928,1687-0247},
   MRCLASS = {05C80 (05E15 20F65)},
MRREVIEWER = {Christian\ Lavault},
       DOI = {10.1093/imrn/rnw287},
       URL = {https://doi.org/10.1093/imrn/rnw287},
}

@article {NguyenTranPlanar,
    AUTHOR = {Nguyen, Hoang Thanh and Tran, Hung Cong},
     TITLE = {On the coarse geometry of certain right-angled {C}oxeter
              groups},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {19},
      YEAR = {2019},
    NUMBER = {6},
     PAGES = {3075--3118},
      ISSN = {1472-2747,1472-2739},
   MRCLASS = {20F65 (20F67)},
MRREVIEWER = {Jiawen\ Zhang},
       DOI = {10.2140/agt.2019.19.3075},
       URL = {https://doi.org/10.2140/agt.2019.19.3075},
}
